An Abaqus UEL implementation of the smoothed finite element method

In this paper, we discuss the implementation of a cell based smoothed finite element method (CSFEM) within the commercial finite element software Abaqus. The salient feature of the CSFEM is that it does not require an explicit form of the derivative of the shape functions and there is no isoparametric mapping. This implementation is accomplished by employing the user element subroutine (UEL) feature of the software. The details on the input data format together with the proposed user element subroutine, which forms the core of the finite element analysis are given. A few benchmark problems from linear elastostatics in both two and three dimensions are solved to validate the proposed implementation. The developed UELs and the associated input files can be downloaded from Github repository link: https://github.com/nsundar/SFEM\_in\_Abaqus.

==> sfemintro.tex <==
In the strain smoothing technique, the compatible strains in the FEM are no longer used to compute the terms in the stiffness matrix. Instead, the integration related to the computation of stiffness matrix is based on the smoothing domain and hence no longer associated with the elements. 

Within the SFEM framework, the discrete modified strain field $\tilde{\varepsilon}_{ij}^h$ that yields the modified strain-displacement matrix $\tilde{\mathbf{B}}$ which is then used to build the stiffness matrix is related to the compatible strain field $\varepsilon_{ij}^h$ by:
\begin{equation}
\tilde {\varepsilon}_{ij}^h (\xx)=\int_{\Omega_C^h}
{\varepsilon _{ij}^h (\xx) ~\bq(\xx) \rmd V }
\label{eqn:epsilonvar}
\end{equation}
where $q(\xx)$ is the smoothing function. On writing \eref{eqn:epsilonvar} at the basis functions derivative level and invoking Gauss-Ostrogradsky theorem, we get:
\begin{equation}
\int_{\Omega_C^h}\phi_{I,x}~\bq(\vm{x})\, \rmd V  =  \int_{\Gamma_C^h}\phi_I~ \bq(\vm{x})n_j\, \rmd S - \int_{\Omega_C^h}\phi_I ~\bq_{,x}(\vm{x})\, \rmd V
\label{eq:divconsistency}
\end{equation}
There are several choices for this smoothing function. For simplicity, $\bq(\xx)$ satisfies the following properties:
\begin{equation}
 \bq \geq0    \hspace{0.2cm} \&    \int\limits_{\Omega^h}\bq(\xx) \rmd \Omega = 1
 \label{eqn:smoothcond}
\end{equation}
In this work, the weighting function, $\bq(\xx)$ is chosen to be a constant, i.e, $\bq(\xx) = 1$ for the simplicity. Using the constant smoothing function ($\bq(\xx)=1$), the modified strains computed using \eref{eq:divconsistency} are constant within the smoothing domain. The Wachspress interpolants are used in this formulation.

%\subsection{Cell based smoothed finite element technique}
In the CSFEM, the local smoothing domain is constructed by sub-dividing the physical element into number of subcells. A subcell for an element is constructed by identifying the centroid\footnote{Here we use the geometric centre of the element.} of the element and connecting the vertices of the polygon/polyhedra with the geometric center of the element. \frefs{fig:csfemsc} - \ref{fig:csfem3dsc} shows the subcells within a polygon and a polyhedra.
\begin{figure}[h!]
\centering
\includegraphics[scale=0.75]{./figures/CSFEMsc.eps}
\caption{Schematic representation of the smoothing cells over arbitrary domain $\Omega$ discretized with arbitrary polygonal finite elements (for example element A-B-C-D-E-F) which are further discretized into the triangular smoothing cells $\Omega_c$ using the centroid of the elements for each element (for example element A-B-C-D-E-F). For interpretation of the colors, the reader is referred to the online version of this article.}
\label{fig:csfemsc}
\end{figure}

\begin{figure}[h!]
\centering
\includegraphics[scale=0.6]{./figures/CSFEM3d.eps}
\caption{Schematic representation of the smoothing cells over polyhedral element (for example element A-B-C-D-E-F-G-H-I-J) which are further discretized into the tetrahedral smoothing cells $\Omega_c$ using the centroid of the elements and its face centroids. For interpretation of the colors, the reader is referred to the online version of this article.}
\label{fig:csfem3dsc}
\end{figure}

Over each subcell, \eref{eq:divconsistency} is evaluated numerically to get the modified strain-deformation matrix. The stiffness matrix computed as for the CSFEM is:
\begin{equation}
\tilde{\mat{K}} = \sum\limits_{I=1}^{nel} \tilde{\mat{K}} = \sum\limits_{I=1}^{nel} \int\limits_{\Omega^e} \tilde{\mat{B}}^\transpose\dd \tilde{\mat{B}}\,\rmd \Omega,
\label{eqn:kmatrix}
\end{equation}
where $\tilde{\mat{B}}$ is the modified strain-displacement matrix. For the chosen smoothing function, the derivative of the function vanishes within the subcell and one integration point (i.e centroid of the smoothing cell $\Omega_c$ denoted by $a$) is sufficient to compute the modified strain-displacement matrix and the corresponding smoothed elemental stiffness matrix. 

Upon substituting the smoothing function, $\bq(\xx) = 1$ in \eref{eq:divconsistency}, the terms in the modified strain-displacement matrix can be computed by:
\begin{equation}
\phi_{a,i} = \dfrac{1}{A_c} \int\limits_{\Gamma_C^h}\phi_a(\vm{x}) n_i\,\rmd S
\label{eq:intconstraints}
\end{equation}
where $i=x,y$ for two dimensions and $i=x,y,z$ for three dimensions, $n_i$ are the unit normals to the edge and face in two and three dimensions, respectively and $A_c$ is the area of the subcell. The above equation for a polygon of $n$ sides, gives the following expression for the modified strain-displacement matrix evaluated at the interior Gauss point:
\begin{equation}
\tilde \bigb=\smat{\tilde {\bigb}_1 &
\tilde {\bigb}_2 & \cdots & \tilde {\bigb}_n} \label{eq:Btilde3dbis},
\end{equation}
where the nodal matrix is
\begin{equation}
\tilde{\bigb}_a =\frac{1}{A_c} \int_{\Gamma_C^h}
\smat{n_x(\xx) & 0 \\
 0 & n_y(\xx) \\
 n_y(\xx) & n_x(\xx) } \phi_a(\xx) \rmd S
\label{eqn:Btilde2d}
\end{equation}
for two dimensions and
\begin{equation}
\tilde{\bigb}_a =\frac{1}{A_c} \int_{\Gamma_C^h}
\smat{n_x(\xx) & 0 & 0\\
 0 & n_y(\xx) & 0\\
 0 & 0 & n_z(\xx) \\
 n_y(\xx) & n_x(\xx) & 0 \\
 0 & n_z(\xx) & n_y(\xx) \\
 n_z(\xx) & 0 & n_x(\xx) } \phi_a(\xx) \rmd S
\label{eqn:Btilde3d}
\end{equation}
for three dimensions. From the above equations, it is clear that only the shape functions are involved in calculating the terms in the stiffness matrix. To evaluate the surface integrals in \eref{eqn:Btilde3d}, we employ the conforming interpolant quadrature technique. 
